ECON: Explicit Clothed humans Optimized via Normal integration

The combination of deep learning, artist-curated scans, and Implicit Functions (IF), is enabling the creation of detailed, clothed, 3D humans from images. However, existing methods are far from perfect. IF-based methods recover free-form geometry, but produce disembodied limbs or degenerate shapes for novel poses or clothes. To increase robustness for these cases, existing work uses an explicit parametric body model to constrain surface reconstruction, but this limits the recovery of free-form surfaces such as loose clothing that deviates from the body. What we want is a method that combines the best properties of implicit representation and explicit body regularization. To this end, we make two key observations: (1) current networks are better at inferring detailed 2D maps than full-3D surfaces, and (2) a parametric model can be seen as a "canvas" for stitching together detailed surface patches. Based on these, our method, ECON, has three main steps: (1) It infers detailed 2D normal maps for the front and back side of a clothed person. (2) From these, it recovers 2.5D front and back surfaces, called d-BiNI, that are equally detailed, yet incomplete, and registers these w.r.t. each other with the help of a SMPL-X body mesh recovered from the image. (3) It "inpaints" the missing geometry between d-BiNI surfaces. If the face and hands are noisy, they can optionally be replaced with the ones of SMPL-X. As a result, ECON infers high-fidelity 3D humans even in loose clothes and challenging poses. This goes beyond previous methods, according to the quantitative evaluation on the CAPE and Renderpeople datasets. Perceptual studies also show that ECON's perceived realism is better by a large margin. Code and models are available for research purposes at econ.is.tue.mpg.de

==> figures/reb-dbni_inputs.tex <==
\newcommand{\dbniInputsCaptionSupMat}{
\cheading{Four inputs to \dbni}
\domainN and \domainD are the domains of clothed and body regions, respectively.
\silhouette is the silhouette of \domainN.
}

\begin{figure}
    \centering
    \vspace{-0.1 em}
    \includegraphics[width=0.8 \linewidth]{photos/dbni_inputs_reb.pdf}
    \vspace{-1.0 em}
    \caption{\dbniInputsCaptionSupMat}
    \vspace{-1.3 em}
\label{fig:dbni_inputs}
\end{figure}

==> figures/reb-errormap.tex <==
\begin{figure}
    \includegraphics[trim=000mm 000mm 000mm 000mm, clip=true, width=1.0\linewidth, height=1cm]{example-image-a}
    \vspace{-1.8 em}
    \caption{
                \cheading{Full error-map, over-smooth back increases error} 
    }
    \vspace{-1.0 em}
    \label{fig: errormap}
\end{figure}



==> figures/reb-speed.tex <==
\begin{figure}
    \includegraphics[trim=000mm 000mm 000mm 000mm, clip=true, width=1.0\linewidth, height=2cm]{example-image-b}
    \caption{
                \cheading{Speed analysis of \pifu, \pamir, \icon and \modelname} 
    }
    \vspace{-1.0 em}
    \label{fig: reb-speed}
\end{figure}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}

==> tabs/dataset.tex <==
\newcommand{\captionDATASETS}{
            Datasets for \threeD clothed humans. 
            Gray color indicates \colorbox{Gray}{datasets} used by \modelname. 
            The bottom ``number of scans'' row indicates the number of scans each method uses.
            The cell format is {\tt ~number\_of\_scans [method]}. 
            \modelname is denoted as {\tt [IC]}. 
            The symbol {\tt $\dagger$} corresponds to the ``8x'' setting in \cref{fig:datasize}.
}

\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|a|a|c|a|}
&\multicolumn{4}{c|}{Train \& Validation Sets}&\multicolumn{2}{c|}{Test Set}  \\  \hhline{~------}
& 
\rotatebox[origin=c]{0}{Renderp.}    & 
\rotatebox[origin=c]{0}{\twindom}    & 
\rotatebox[origin=c]{0}{\agora}      & 
\rotatebox[origin=c]{0}{\thuman}     & 
\rotatebox[origin=c]{0}{\buff}       & 
\rotatebox[origin=c]{0}{\cape}       \\ 
& 
\cite{renderpeople}         & 
\cite{twindom}              & 
\cite{patel2021agora}       & 
\cite{zheng2019deephuman}   & 
\cite{zhang2017buff}        &  
\cite{ma2020cape,ponsMoll2017clothCap}\\
\shline
Free \& public     &   \xmark   &   \xmark    &  \xmark    &   \cmark   &   \cmark    &    \cmark \\ 
Diverse poses      &   \xmark   &   \xmark    &  \xmark    &   \cmark   &   \xmark    &    \cmark \\ 
Diverse identities &   \cmark   &   \cmark    &  \cmark    &   \xmark   &   \xmark    &    \xmark \\ 
SMPL(-X) poses     &   \xmark   &   \xmark    &  \cmark    &   \cmark   &   \cmark    &    \cmark \\ 
High-res texture   &   \cmark   &   \cmark    &  \cmark    &   \xmark   &   \cmark    &    \cmark \\ 
\hline
\multirow{3}{*}{Number of scans} & \multicolumn{1}{l|}{450~\cite{saito2019pifu,saito2020pifuhd}} & 1000~\cite{zheng2020pamir} & ~~450~[IC] & ~~600~[$\text{IC}^{\dagger}$]  & ~~~~~5~\cite{saito2019pifu,saito2020pifuhd} & 150~[IC] \\
\qquad \quad  & \multicolumn{1}{l|}{375~\cite{huang2020arch}} & & ~3109~[$\text{IC}^{\dagger}$] & ~600~\cite{zheng2020pamir} & \multicolumn{1}{l|}{~~~26~\cite{huang2020arch}} & \\
& & & & & \multirow{1}{*}{~300~\cite{zheng2020pamir,li2020realtimeVolMoCap}} & \\
\end{tabular}
}
\vspace{-0.5 em}
\caption{\captionDATASETS}
\vspace{-0.3 em}
\label{tab:dataset}
\end{table}


==> tabs/multi-normal.tex <==
\begin{table}[H]
\vspace{-1.3 em}
\centering{
\resizebox{0.45\textwidth}{!}{
  \begin{tabular}{c|cccc|cccc}
    Methods & \multicolumn{4}{c|}{OOD poses (\cape)} 
     & \multicolumn{4}{c}{OOD outfits (\renderppl)}\\
    Normal $\downarrow$ & $0^\circ$ (front) & $90^\circ$ & $180^\circ$ (back) & $270^\circ$
     & $0^\circ$ (front) & $90^\circ$ & $180^\circ$ (back) & $270^\circ$ \\
    \shline
    $\text{\modelname}$ & 0.024 &  0.049 &  0.022 &  0.036 & 0.032 & 0.091 & 0.023 & 0.062 \\
  \end{tabular}}
}
\vspace{-1.0 em}
\caption{
    \cheading{Cross-view ``Normal'' error of \modelname}}
\vspace{-1.2 em}
\label{tab:multi-normal}
\end{table}


